Learning Robust Representations via Multi-View Information Bottleneck

The information bottleneck principle provides an information-theoretic method for representation learning, by training an encoder to retain all information which is relevant for predicting the label while minimizing the amount of other, excess information in the representation. The original formulation, however, requires labeled data to identify the superfluous information. In this work, we extend this ability to the multi-view unsupervised setting, where two views of the same underlying entity are provided but the label is unknown. This enables us to identify superfluous information as that not shared by both views. A theoretical analysis leads to the definition of a new multi-view model that produces state-of-the-art results on the Sketchy dataset and label-limited versions of the MIR-Flickr dataset. We also extend our theory to the single-view setting by taking advantage of standard data augmentation techniques, empirically showing better generalization capabilities when compared to common unsupervised approaches for representation learning.

==> figures/model.tex <==



==> sections/app_general_objective.tex <==
The Multi-View Information Bottleneck objective can be seen as a more general version of Variational Information Bottleneck \citep{Alemi2016}, InfoMax and Multi-View InfoMax\citep{Ji2018, Henaff2019, Tian2019, Bachman2019} families of objectives:


\paragraph{Multi-View InfoMax} Setting $\beta=0$ completely disregards the requirement for minimality of the representation with respect to the second view.
In this setting, the MIB loss correspond to mutual information maximization across views:
\begin{align*}
    \gL_{MIB(\text{MV-InfoMax})}(\theta,\psi;0) = -I_{\theta\psi}(\rvz_1;\rvz_2).
\end{align*}

\paragraph{InfoMax} By picking $\rvv_1=\rvx$ and $\rvv_2=\rvx$, the MIB objective degenerates to information maximization. This is because whenever $p_\theta(\rvz_1|\rvv_1)$ and $p_\psi(\rvz_2|\rvv_2)$ share their parameter, they represent exactly the same distribution (since $\rvv_1=\rvv_2=\rvx$).
As a consequence, the Symmetrized KL-divergence between the two posteriors is always 0:
\begin{align*}
    \gL_{MIB(\text{InfoMax})}(\theta) = -I_{\theta}(\rvz_1;\rvz_2).
\end{align*}
Note that the dependency on $\beta$ and $\psi$ are dropped, while the maximization of $I_{\theta}(\rvz_1;\rvz_2)$ becomes equivalent to $I_\theta(\rvx;\rvz)$.

\paragraph{Variational information bottleneck} Selecting the observations as the first view and the label as the second one, we obtain the same trade-off between sufficiency and minimality reported in the VIB loss function:
\begin{align*}
    \gL_{MIB(\text{VIB})}(\theta,\psi;\beta) = -I_{\theta\psi}(\rvz_1;\rvz_2) + \beta D_{SKL}(p_\theta(\rvz_1|\rvx)||p_\psi(\rvz_2|\rvy)),
\end{align*}
where the first term is equivalent to maximizing $I(\rvz;\rvy)$ while the second one corresponds to the minimization of $I(\rvx;\rvz)$.
Although, the two models differ for the strategy used for the optimization procedure and approximations.

Depending on the amount of information the two views have in common, the MIB objective can interpolate between InfoMax (all information is shared across the two views) and Variational Information Bottleneck (only the label information is share across the two views).

==> sections/method.tex <==
\section{Exploiting multiple data-views in Theory}
\label{sec:method}
% First of all, any representation that contains all the information about the original observations is as useful as the original data itself. 
% On the other hand, such a representation would not be invariant to any nuisance of the task by definition.
% In this work we show that is possible to exploit some properties of the task to obtain a smaller (more invariant) representation that does not violate the sufficiency constrain even when the target $Y$ is not available.\\\\
% \todo{This is an example to introduce the side information}

% Enforcing sufficiency and minimality directly can be done only in supervised settings, since the label $\rvy$ needs to be observed. In this section, we show that it is possible to obtain a robust data representation by exploiting some known properties of the task in weakly and self-supervised settings.

Let $\rvv_1$ and $\rvv_2$ be two images of the same object from different view-points and let $\rvy$ be its label.
Assuming that the object is clearly distinguishable from both $\rvv_1$ and $\rvv_2$, any representation $\rvz$ with all the information that is accessible from both views would also contain the necessary label information. Furthermore, if $\rvz$ captures only the details that are visible from both pictures, it would reduce the total information content, discarding the view-specific details and reducing the sensitivity of the representation to view-changes.
The theory to support this intuition is described in the following where $\rvv_1$ and $\rvv_2$ are jointly observed and referred to as data-views.


\subsection{Redundancy and Sufficiency}
%Let $\rvv_1$ and $\rvv_2$ be the two observed data-views and $\rvy$ the associated target label.
We consider relations between the three random variables starting by formally defining \textbf{redundancy}.
\begin{definition}{Redundancy:}
 $\rvv_1$ is redundant with respect to $\rvv_2$ for $\rvy$ if and only if $I(\rvy;\rvv_1|\rvv_2)=0$ 
\end{definition}
Intuitively, a view $\rvv_1$ is redundant for a task whenever it is irrelevant for the prediction of $\rvy$ when $\rvv_2$ is already observed.
In this scenario,  $\rvv_2$ contains all the information needed for the task, therefore any representation $\rvz_1$ of $\rvv_1$ sufficient for $\rvv_2$ must be as predictive as $\rvv_1$ itself:

% \textcolor{yellow}{
% We formalize the concept of \textbf{non-complementarity} to specify contexts in which the two views contain the same information regarding the label $\rvy$
% \begin{definition}{Non-complementarity:}
% Two random variables $\rvx$ and $\rvw$ are not complementary with respect to $\rvy$ if and only if $\rvx$ is redundant with respect to $\rvw$ for $\rvy$ and $\rvw$ is redundant with respect to $\rvx$ for $\rvy$.
% \end{definition}
% Intuitively, two views are non-complementary whenever the uncertainty on the prediction of the target does not increase if either one of the two is observed instead of their joint occurrence.
% Note that, whenever $\rvy$ is discrete, assuming that the label is uniquely identifiable from both views is a stricter condition than non-complementarity\todo{Is the proof needed?}. 
% \\\\
% Whenever $\rvx$ and $\rvw$ are known to be non-complementary, it is possible to guarantee sufficiency of their joint representation by ensuring that the representation of one of them contains all the information that that is shared across the two views: 
% \begin{theorem}
% \label{th:main}
%     Let $\rvx$ and $\rvw$ be two non-complementary views with respect to $\rvy$.
%     Any representation $\rvz$ of $\rvx$ that is sufficient for $\rvw$ is also sufficient for $\rvy$ 
% \end{theorem}}
\begin{customlemma}{\ref{lemma:multi_suff}}
    Let $\rvv_1$ be redundant view with respect to $\rvv_2$ for $\rvy$.
    Any representation $\rvz_1$ of $\rvv_1$ that is sufficient for $\rvv_2$ is also sufficient for $\rvy$ 
\end{customlemma}
Notably, Lemma~\ref{lemma:multi_suff} imposes a restriction on the representation $\rvz_1$ that does not depend on $\rvy$, guaranteeing sufficiency for the target even when the label is not observed.
Nevertheless, there are no guarantees that $\rvv_1$ is as predictive as $\rvv_2$ for $\rvy$ in the first place. In fact, when both views are observed, one could build a model that considers $\rvv_1$ and $\rvv_2$ together to better predict $\rvy$.

Whenever $\rvv_1$ and $\rvv_2$ contain the same information regarding the target ($\rvv_1$ is redundant with respect to $\rvv_2$, and vice-versa), it is possible to extend the result of Lemma~\ref{lemma:multi_suff}:

\begin{customcorollary}{\ref{cor:suff_multi}}
Let $\rvv_1$ and $\rvv_2$ be two mutually redundant views for a target $\rvy$. Any representation $\rvz_1$ of $\rvv_1$ that is sufficient for $\rvv_2$ is as predictive for $\rvy$ as the joint observation of the two views.
\end{customcorollary}
In other words, whenever it is possible to assume mutual redundancy, any representation of one view containing all the information regarding the other view is as useful as both views for predicting the label $\rvy$. 
The proofs and formal statements for Lemma~\ref{lemma:multi_suff} and Corollary~\ref{cor:suff_multi} are in Appendix \ref{app:proofs}.
% \anjan{Theorem and Corollary both should start from 1}

\subsection{Minimality and Independence}
Any encoder that replicates $\rvv_1$ in $\rvv_2$ satisfies the sufficiency condition in Lemma~\ref{lemma:multi_suff}, but is not generalizable \citep{Tschannen2019}.
Similar to the single-view setting, we can show that minimality of $\rvz_1$ for $\rvv_2$ yields invariance to some nuisances of the target influencing the raw observations.

% \textcolor{blue}{In order to better understand what information is retained through the encoding procedure, one can subdivide $I(\rvv_1;\rvz_1)$ into three components by using the chain rule of mutual information (see Appendix~\ref{app:chain}):
% \begin{align}
% \label{eq:decomposition}    
% I(\rvv_1;\rvz_1) &= \underbrace{I(\rvv_1;\rvz_1|\rvv_2)}_{\text{$\rvv_1$-private information}} + \underbrace{I(\rvv_1;\rvv_2)}_{\text{shared-information}}- \underbrace{I(\rvv_1;\rvv_2|\rvz_1)}_{\text{shared-information not in $\rvz_1$}} 
% \end{align}
% The conditional mutual information $I(\rvv_1;\rvz_1|\rvv_2)$ will be referred to as the $\rvv_1$\textbf{-private} information since it represents the amount of information in $\rvz_1$ that can not be predicted from $\rvv_2$. The second term $I(\rvv_1;\rvv_2)$ is a constant determined by how much information the two views have in common; while the last term $I(\rvv_1;\rvv_2|\rvz_1)$ represents the amount of information regarding $\rvv_2$ that is lost by encoding $\rvv_1$ into $\rvz_1$. Note that this last term is zero whenever $\rvz_1$ is sufficient for $\rvv_2$.
% By considering the three terms in Equation~\ref{eq:decomposition}, one can notice that the minimum amount of information that needs to be represented in $\rvz_1$ without violating the sufficiency constrain for $\rvv_2$ is the common information between the two views $I(\rvv_1;\rvv_2)$.
% Furthermore, since mutual information is always positive, $I(\rvv_1;\rvz_1)$ is minimal only when $I(\rvv_1;\rvz_1|\rvv_2)=0$. This is true whenever $\rvz_1$ discards all the $\rvv_1$-private information and, therefore, the representation $\rvz_1$ is minimal with respect to $\rvv_2$.}
% \begin{definition}{$\rvx$-private representation:}
% A representation $\rvz$ of a view $\rvx$ is $\rvx$-private with respect to a second view $\rvw$ if and only if $I(\rvz_x;\rvw)=0$
% \end{definition}
% \begin{definition}{Minimality (multi-view):}
% A representation $\rvz$ of a view $\rvx$ is minimal with respect to $\rvw$ whenever is does not contain any $\rvx$-private information.
% \end{definition}
% \begin{remark}
% Since $Z$ is a representation of $X$ it is also independent of any $W$-private nuisances.
% \end{remark}
% Therefore, the minimality of a sufficient representation $Z$ can be re-defined as:
% \begin{definition}{Minimality (Multi-view):}
% \label{def:minmult}
% A representation $Z$ of a view $X$ is minimal with respect to a second view $W$ whenever $I(X;Z|W)=0$.
% \end{definition}

Whenever the two views are mutually redundant for predicting $\rvy$, the information that can be accessed from only one view must be irrelevant for the task since if only one view contains some crucial information, that view would not be redundant for predicting $\rvy$. This violates the redundancy assumption (Theorem~\ref{th:label_idependence}). Such superfluous information is also discarded by any $\rvz_1$ of $\rvv_1$ that is exclusive for $\rvv_2$ (Corollary~\ref{cor:multi_nuisances}).
% \begin{customcorollary}{\ref{cor:multi_nuisances}}
% Let $\rvv_1$ and $\rvv_2$ be mutually redundant views for $\rvy$.
% Let $\rvn$ be a random variable that is independent of $\rvv_2$. Any representation $\rvz_1$  of $\rvv_1$ that is exclusive for $\rvv_2$ is independent of $\rvn$.
% \end{customcorollary}
% Note all the nuisances $\rvn$ of $\rvx$ that do not correlate with $\rvw$ are discarded during the encoding procedure.
%
% In other words, by enforcing exclusivity of the representation for $\rvv_2$, any information in $\rvv_1$ that is not predictable from $\rvv_2$ is discarded. 
Furthermore, since $\rvz_1$ depends only on $\rvv_1$, the representation does not contain any information accessible only from $\rvv_2$ (Corollary~\ref{cor:multi_nuisances}). 
The less the two views have in common, the more information can be safely discarded without violating sufficiency for $\rvy$.

\subsection{Self-supervision and Invariance}
\label{subsec:augmentation}
% On one hand, a representation of one view $\rvx$ that is both minimal and sufficient for another view $\rvw$ carries the same amount of information regarding the target while being more robust to nuisances then the original data.
% In theory, by enforcing the sufficiency and minimality conditions it is possible to obtain a representation that is as discriminative as the original data while being more robust to nuisances.
%In practice, it may be difficult to obtain data-views that satisfy the mutual redundancy condition.
In this section, we introduce a methodology to build mutually redundant views starting from single observations $\rvx$ with domain $\sX$ by exploiting known symmetries of the task. 

By picking a class $\sT$ of functions $t:\sX \to \sW$ that do not affect label information, it is possible to artificially build views that satisfy mutual redundancy for $\rvy$ with a procedure similar to data-augmentation.
Let $\rvt_1$ and $\rvt_2$ be two random variables over $\sT$, then $\rvv_1:=\rvt_1(\rvx)$ and $\rvv_2:=\rvt_2(\rvx)$ must be mutually redundant for $\rvy$ (Corollary~\ref{th:mutual_redundance_augmentation}).
Since no function in $\sT$ affects label information ($I(\rvv_1;\rvy)=I(\rvv_2;\rvy)=I(\rvx;\rvy)$), a representation $\rvz_1$ of $\rvv_1$ that is sufficient to $\rvv_2$ must contain same amount of predictive information as $\rvx$ (Corollary~\ref{th:suff_augmentation}). 

Whenever the two transformations for the same observations are independent ($I(\rvt_1;\rvt_2|\rvx)=0$), they introduce uncorrelated variations in the two views. As an example, if $\sT$ represents a set of small translations, the two views will differ by a small shift. Since this information is not shared, $\rvz_1$ that contains only common information between $\rvv_1$ and $\rvv_2$ will discard fine-grained details regarding the position. Further details regarding the characteristics of the function class and connection to the literature on invariance can be found in Appendix~\ref{app:invariance}.



% \begin{definition}{$\rvt$-Invariance:}
% Let $\sT$ be a class of functions $t:\sX \to \sW$.
% Let $\rvx$, $\rvy$ and $\rvt$ be random variables with domain $\sX$, $\sY$ and $\sT$ respectively and joint distribution $p(\rvx)p(\rvy|\rvx)p(\rvt|\rvx)$. The conditional distribution $p(\rvy|\rvx)$ is $\rvt$-invariant if and only if $p(\rvy|\rvx)=p(\rvy|\rvt(\rvx))$.
% \end{definition}

% Whenever the predictive task is known to be invariant with respect to a function class $\sT$, it is possible to define a second view by applying a random $t\in\sT$ to the observations $\rvx$ and produce a second view $\rvv_2= \rvt(\rvx)$ that carries the same information about the label.
% Since the information regarding $\rvy$ is not discarded by applying any $t\in\sT$, the resulting view must be mutually redundant with respect to $\rvx$.

% \begin{lemma}
% \label{lemma:invariance}
% Let $\sT$ be a class of functions $t:\sX\to\sW$.
% Let $\rvx$, $\rvy$ and $\rvt$ be random variables with joint distribution $p(\rvx)p(\rvy|\rvx)p(\rvt|\rvx)$ and support $\sX$, $\sY$ and $\sT$ respectively, then $\rvx$ and $\rvt(\rvx)$ are mutually redundant for $\rvy$ if and only if $p(\rvy|\rvx)$ is $\rvt$-invariant.
% \end{lemma}

% In other words, whenever a second data-view is built by applying $\rvt$ to the raw observations $\rvx$, mutual redundancy of the two views and $\rvt$-invariance are equivalent.
% Using the result from Theorem~\ref{th:independence} one can show that exclusivity of a representation $\rvz$ of $\rvx$ for $\rvt(\rvx)$ is equivalent to $\rvt$-invariance of the encoding distribution $p(\rvz|\rvx)$:

% \begin{corollary}
% \label{cor:invariance}
% Let $\sT$ be a class of functions $t:\sX\to\sW$.
% Let $\rvx$ and $\rvt$ be random variables with joint distribution $p(\rvx,\rvt)$ and support $\sX$ and $\sT$ respectively. A representation $\rvz$ of $\rvx$ is exclusive for $\rvt(\rvx)$ if and only if $p(\rvz|\rvx)$ is $\rvt$-invariant.
% \end{corollary}

% An alternative procedure to build mutually redundant views consists creating the two views $\rvv_1$ and $\rvv_2$ by applying randomly selected functions in $\sT$ to the same observation. Analogously to the previously described scenario, exclusivity of a representation $\rvz_1$ of $\rvv_1$ implies $\rvt$-invariance and sufficiency of $\rvz$ for $\rvv_2$ implies $I(\rvz;\rvy)=I(\rvx;\rvy)$.

% \textcolor{blue}{
% Rewrite this section in a more practical perspective
% }
% \begin{figure}
%     \centering
%     \includegraphics[draft]{figures/transform.pdf}
%     \caption{Figure to show how to build the mutually redundant views}
%     \label{fig:transforms}
% \end{figure}

%\begin{corollary}
%Let $\rvx$ and $\rvy$  be random variables with support $\sX$ and $\sY$ respectively.
%A representation $\rvz$ of $\rvx$ is sufficient for $\rvy$ if and only if $p(\rvy|\rvx)$ is invariant to $\gE:=\left\{e:\sX\to\sZ| p(\vx,e(\vx))>0 \right\}$.
%\end{corollary}

% Any function of $\rvx$ must be redundant for predicting the label $\rvy$ by construction since no new information in introduced. Let $T: \sX \times \sK \to \sW$ be a transformation of $\rvx$ dependent on some independently distributed parameters $\rvk\in\sK$ and let $\rvw=T(\rvx,\rvk)$.
% Whenever $T$ does not destroy any label information for any parameter $k\in\sK$, $\rvw$ must also be as predictive for $\rvy$ as $\rvx$ ($I(\rvw;\rvy)=I(\rvx;\rvy)$). Therefore the transformed observation $\rvw$ must be a mutually redundant view with respect to $\rvx$ for $\rvy$.\todo{statement and proof in the appendix}

% Since the mutual redundancy relation is transitive\todo{proof}, by defining two transformations $T_1:\sX\times\sK_1\to\sW_1$ and $T_2:\sX\times\sK_2\to\sW_2$, it is possible to create mutually redundant views $\rvw_1=T_1(\rvx,\rvk_1)$ and $\rvw_2=T_2(\rvx,\rvk_2)$ on the condition that both transformations preserve the label information.

% \begin{figure}
%     \centering
%     \includegraphics[draft]{figures/visualization.png}
%     %\input{figures/diagram_1.tex}
%     \caption{
%     TODO decide what figure can help to explain and put it here
%     % Visualization of the minimal sufficient representation $\rvz$ for a binary classification problem. The two views $\rvv\in\sV$ and $\rvw\in\sW$ are respectively obtained by applying the stochastic transformations $T_v: \sX \times \sK_v \to \sV$ and $T_w: \sX \times \sK_w \to \sW$ to the observation $\rvx\in\sX$. Since $T_v$ and $T_w$ must preserve the label information (here denoted with different colors), the images of $\left\{ x_1, x_2\right\}$ and $\left\{ x_3\right\}$ must be disjoint in both $\sV$ and $\sW$. As a consequence, the images $e(\left\{v_1,v_2\right\})$ and $e(\left\{v_3,v_4\right\})$ determined bu the encoder $e: \sV \to \sZ$ must also be disjoint sets whenever $\rvz$ is sufficient for $\rvw$. Since $\rvv$ and $\rvw$ rely on independent sources of stochasticity, any representation $\rvz$ that is minimal for $\rvw$ must collapse $v_1$ and $v_2$ to the same point.
%     } 
%     \label{fig:theory}\todo{update}
% \end{figure}
% Expressing $X=T(W,\theta)$, we can create one view as any transformation $T$ of the observed data $W$ that depends on some parameters $\theta$. 
% Whenever it is known that $T$ does not affect the target information for every $\theta$ and $W$, it can be used to artificially create a second view $X$ that satisfies the non-complementarity condition for the task.
% Whenever the parameters of the transformations $\rvk_1$ and $\rvk_2$ independent of each other, $I(\rvw_1;\rvk_2)$ must be zero. Therefore, any representation $\rvz$ of $\rvw_1$ that is minimal for $\rvw_2$ is invariant to the parameters of the transformation (Theorem~\ref{th:invariance}):
% \begin{corollary}
% \label{co:inv}
%     Let $\rvx$ and $\rvk$ be independent random variables.
%     Let $\rvw=T(\rvx,\rvk)$ for some function $T: \sX\times\sK\to\sW$.
%     A representation $\rvz$ of $\rvw$ is minimal with respect to $\rvx$ if and only $p(\rvz|\rvw)$ is symmetric with respect to $T$.
% \end{corollary}

% Corollary~\ref{co:inv} guarantees that any minimal representation $\rvz$ is invariant to the parameters of the transformation.
% More precisely, if $x_1$ and $x_2$ can be represented as the transformation of the same $w$ for two different $\theta_1\neq\theta_2$, they must be associated to the same representation $f(x_1,\eta)=f(x_2,\eta)$.
% By considering transformations that have image $\mathcal{W}$ ( $T:\mathcal{W}\times\Theta\to\mathcal{W}$ ) for which there exist a $\theta_{Id}$ that corresponds to the identity on $\mathcal{W}$ ( $W=T(W,\theta_{Id})$ ), it is possible to build a representation $Z$ that is constant on the orbits defined by $T$.
% \todo{explain more and formalize better}

% In particular, by defining $T$ as a group action, and identifying $\theta$ as group elements $g\in\mathcal{G}$, the minimal representation of $X$ for $W$ must be invariant to $\mathcal{G}$.

% \textcolor{blue}{
%     \begin{enumerate}
%         \item Connection to group theory by defining $W=f(X, \theta)$ \citep{2019arXiv190106082B}
%     \end{enumerate}
% }


==> tables/flickr_example_simple.tex <==
\begin{tabular}{c c c}
     $\rvv_1$ & $ \rvv_2$ & $\rvy$  \\\hline
     \parbox{0.25\textwidth}{\vspace{0.1cm} \includegraphics[width=0.24\textwidth]{figures/dog_flickr.png}\vspace{0.1cm}} & \parbox{0.3\textwidth}{\centering\tiny ``watermelon'', ``hilarious'', ``dog''} & 
     \parbox{0.3\textwidth}{\centering\tiny
      ``dog'', ``food'', ``animals''}\\
     \parbox{0.25\textwidth}{\vspace{0.1cm}\includegraphics[width=0.24\textwidth]{figures/building_flickr.png}\vspace{0.1cm}} & \parbox{0.3\textwidth}{\centering\tiny ``colors'', ``cores'', ``centro'', ``building''} & \parbox{0.3\textwidth}{\centering\tiny
     ``clouds'', ``sky'', ``structures''}
\end{tabular}

==> tables/flickr_results_simple.tex <==
\begin{tabular}{ll}
    Method          & mAP   \\ \hline
    Original Inputs & 0.48  \\
    CCA             & 0.529 \\
    % Contrastive \citep{Hermann2013} & 0.565 \\
    DCCA \citep{Galen13}            & 0.573 \\
    % DCCAE \citep{Wang2016} & 0.573\\
    MVAE-var \citep{Ngiam2011} & 0.595 \\
    bi-VCCA-private \citep{Wang2016} & 0.626 \\\hline
    \textbf{MV-InfoMax}       & \textbf{0.751} \\
    \textbf{MIB} ($\beta=10^{-3}$)       &  \textbf{0.749} \\
    MIB ($\beta=1$)       &  0.688
\end{tabular}

==> tables/mnist_example.tex <==
\begin{tabular}{c c c}
     $\rvv_1\in[0,1]^{28\times28}$& $\rvv_2\in[0,1]^{28\times28}$ & $\rvy\in[10]$  \\\hline
      \parbox{0.3\textwidth}{\vspace{0.1cm}\includegraphics[width=0.3\textwidth]{figures/mnist_11.png}\vspace{0.1cm}} &  \parbox{0.3\textwidth}{\includegraphics[width=0.3\textwidth]{figures/mnist_12.png}} &
     \parbox{0.2\textwidth}{\centering ``3''}\\
     \parbox{0.3\textwidth}{\vspace{0.1cm}\includegraphics[width=0.3\textwidth]{figures/mnist_21.png}\vspace{0.1cm}} &  \parbox{0.3\textwidth}{\includegraphics[width=0.3\textwidth]{figures/mnist_22.png}} &  \parbox{0.2\textwidth}{\centering
         ``6''}
\end{tabular}

==> tables/mnist_example_simple.tex <==
\begin{tabular}{c c c}
     $\rvv_1$& $\rvv_2$ & $\rvy$  \\\hline
      \parbox{0.25\textwidth}{\vspace{0.1cm}\includegraphics[width=0.25\textwidth]{figures/mnist_11.png}\vspace{0.1cm}} &  \parbox{0.25\textwidth}{\includegraphics[width=0.25\textwidth]{figures/mnist_12.png}} &
     \parbox{0.25\textwidth}{\centering ``3''}\\
     \parbox{0.25\textwidth}{\vspace{0.1cm}\includegraphics[width=0.25\textwidth]{figures/mnist_21.png}\vspace{0.1cm}} &  \parbox{0.25\textwidth}{\includegraphics[width=0.25\textwidth]{figures/mnist_22.png}} &  \parbox{0.25\textwidth}{\centering
         ``6''}
\end{tabular}

==> tables/sketchy_example_simple.tex <==
\begin{tabular}{c c c}
     $\rvv_1$& $\rvv_2$ & $\rvy$  \\\hline
      \parbox{0.25\textwidth}{\vspace{0.1cm}\includegraphics[width=0.25\textwidth]{figures/cat_picture.jpg}\vspace{0.1cm}} &  \parbox{0.25\textwidth}{\includegraphics[width=0.25\textwidth]{figures/cat_sketch.png}} &
     \parbox{0.25\textwidth}{\centering ``cat''}\\
     \parbox{0.25\textwidth}{\vspace{0.1cm}\includegraphics[width=0.25\textwidth]{figures/apple_picture.jpg}\vspace{0.1cm}} &  \parbox{0.25\textwidth}{\includegraphics[width=0.25\textwidth]{figures/apple_sketch.png}} &  \parbox{0.25\textwidth}{\centering
         ``apple''}
\end{tabular}


==> tables/sketchy_results_simple.tex <==
\begin{tabular}{lll}
            Method                                                    & mAP@all & Prec@200 \\ \hline
            % SaN \citep{Qian2015}                                                    & 0.208   & 0.292    \\
            GN Triplet \citep{Sangkloy2016}                                              & 0.529   & 0.716    \\
            % Siamese CNN                                              & 0.481   & 0.612    \\
            Siamese-AlexNet \citep{Qi2016}                                        & 0.518   & 0.690    \\
            Triplet-AlexNet                                          & 0.573   & 0.761    \\
            DSH$^{*}$ \citep{Liu2017} & 0.711   & \textbf{0.866}    \\
            GDH$^*$ \citep{Zhang2018} & 0.810   & -        \\\hline
            
            %MV-InfoMax\addtocounter{footnote}{1}\addtocounter{footnotesintable}{1}\footnotemark[\thefootnote]& 0.008  &  0.008    \\

            % MV-InfoMax$^\ref{note:1}$ & 0.008  &  0.008    \\
            \textbf{MIB }& \textbf{0.856}  &  0.848   \\
            MIB$^*$ (64-bits)                                         &  0.851   & 0.834  
        \end{tabular}
